Weakly-supervised Contextualization of Knowledge Graph Facts

Knowledge graphs (KGs) model facts about the world, they consist of nodes (entities such as companies and people) that are connected by edges (relations such as founderOf). Facts encoded in KGs are frequently used by search applications to augment result pages. When presenting a KG fact to the user, providing other facts that are pertinent to that main fact can enrich the user experience and support exploratory information needs. KG fact contextualization is the task of augmenting a given KG fact with additional and useful KG facts. The task is challenging because of the large size of KGs, discovering other relevant facts even in a small neighborhood of the given fact results in an enormous amount of candidates. We introduce a neural fact contextualization method (NFCM) to address the KG fact contextualization task. NFCM first generates a set of candidate facts in the neighborhood of a given fact and then ranks the candidate facts using a supervised learning to rank model. The ranking model combines features that we automatically learn from data and that represent the query-candidate facts with a set of hand-crafted features we devised or adjusted for this task. In order to obtain the annotations required to train the learning to rank model at scale, we generate training data automatically using distant supervision on a large entity-tagged text corpus. We show that ranking functions learned on this data are effective at contextualizing KG facts. Evaluation using human assessors shows that it significantly outperforms several competitive baselines.

==> distant-sup.tex <==
%!TEX root = ./main.tex
\section{Gathering noisy training data}
\label{sec:distance-supervision}
\NV{Restructure this}
We follow the distant supervision paradigm to automatically gather training data~\cite{mintz2009distant}. 
%
The knowledge graph we use is tightly integrated with Wikipedia, therefore we use Wikipedia articles to find relevant facts to a relationship.
%
We treat the main entity $e$ of a Wikipedia article as the source entity, and follow the procedure below.
%
First, we augment Wikipedia articles with dense entity links, as in~\cite{voskarides-generating-2017}.
%

%
The procedure we follow is outlined in Algorithm \ref{alg:data-extraction} \NV{Update this algorithm}. The assumption is that sentence in the article of the main entity that mentions another entity expresses the relation between the main entity and the other entity~\cite{voskarides-generating-2017}.
%
%
\begin{algorithm}[t]
\caption{Training instances extraction for entity $e$  \NV{UPDATE: see possible settings}}
\label{alg:data-extraction}
\begin{algorithmic}[1]
\Require{A knowledge graph $K$, Wikipedia corpus $W$, entity $e$ (e.g. Bill Gates)}
%
\Ensure{A set of training instances $X$}
\State $a \gets$ \textproc{GetWikipediaArticle($W, e$)}
\State $T \gets \{\}$  \Comment{Keeps track of entities directly connected to $e$}
\State $X \gets \{\}$   \Comment{  $\langle r(e, ?),  listoftriples\rangle$ }
\For{$s \in a$}  \Comment{For each sentence/paragraph}
	\State $s' \gets$ \textproc{DenseEntityLinking($s, e, W, K$)} \Comment{Including dates}
	%
    \State $E \gets$  \textproc{GetEntities($s$)} $\setminus \{e\}$  \Comment{Excluding entity $e$}
    %
    \If{$|E| < 2$}
    	%
        \State continue \Comment{Only one other entity, so no context+}
		%
    \EndIf
    %
    %
    \For{$t \in E$}  \Comment{For each other entity}
		%
        \If{$t \in T$} \Comment{entity already selected (we only care about first appearances of entities in the Wikipedia article~\cite{voskarides-generating-2017})}
        	\State continue
        \EndIf
        %
        \State $z \gets$ \textproc{DirectRelations($e, t, K$)}  \Comment{$r_i(e, t)$}
        %
        \If{$|z| \neq 1$}  \Comment{there exists more than a single direct relation between $e$ and $e'$, therefore the relation expressed is ambiguous (we only care about  unambiguous relations~\cite{sorokin2017context})}
			\State continue        
        \EndIf

        %
        \State $T.add(t)$  \Comment{Bookkeeping}
        %
        \State $x \gets \{ \}$
        %
        \State $x.add(z)$
        %
        \For{$ \langle a, b \rangle \in$ \textproc{GeneratePairs($E \cup \{e\}$)}} \Comment{For all pairs of entities in $E$ and $e$}
        %
        \State $z' \gets$ \textproc{DirectRelations($a, b, K$)} 
        %
        \If{$z = z' \vee |z'| \neq 1$}  \Comment{already added in $x$ or ambiguous relation}
        \State continue 
        \EndIf
        %
        \State $x.add(z')$
        %
        \EndFor
        %
        \If{$|x| > 1$}  \Comment{More than one triple}
        \State $X.add(x)$
        \EndIf
        %
    %
    \EndFor
    %
\EndFor
%
\State \Return $X$
\end{algorithmic}
\end{algorithm}
%

Motivation Examples
\begin{itemize}
	\item $\mathit{FounderOf}(\mathit{Bill Gates}, \mathit{Microsoft})$:     ``In 1975, Gates and Paul Allen launched Microsoft, which became the world's largest PC software company.''
    \begin{itemize}
    	\item $\langle Microsoft, FoundingDate, 1975 \rangle$
        \item $\langle Paul Allen, FounderOf, Microsoft \rangle$
        \item $\langle Microsoft, Type, Company \rangle$
        \item $\langle Software, IndustryOf, Microsoft \rangle$
    \end{itemize}
    \item $\mathit{spouseOf}(\mathit{Bill Gates}, \mathit{Melinda Gates})$: ``Bill Gates married Melinda French on a golf course on the Hawaiian island of Lanai January 1, 1994; he was 38 and she was 29. They have three children: Jennifer Katharine, Rory John, and Phoebe Adele.''
    \begin{itemize}
    	\item $\langle spouseMed, Start date, 01/01/1994 \rangle$
        \item $\langle Bill Gates, ParentOf, Jennifer Katharine Gates \rangle$  
        \item $\langle Bill Gates, ParentOf, Rory John Gates \rangle$
        \item $\langle Bill Gates, ParentOf, Phoebe Adele \rangle$
        \item $\langle Melinda Gates, ParentOf, Jennifer Katharine Gates \rangle$  
        \item $\langle Melinda Gates, ParentOf, Rory John Gates \rangle$
        \item $\langle Melinda Gates, ParentOf, Phoebe Adele \rangle$
        \item $\langle Bill Gates, DateOfBirth, 1955 \rangle$  \NV{needs logic to extract}
        \item $\langle Melinda Gates, DateOfBirth, 1964 \rangle$  \NV{needs logic to extract}
    \end{itemize}
    
\end{itemize}


Table~\ref{tab:distant-supervision-settings} shows possible settings of the distant supervision extraction procedure \NV{Remove table and keep the setting we used (least aggressive filtering strategy)}.
\begin{table}[t]
\small
\caption{Distant supervision settings}
\label{tab:distant-supervision-settings}
\vspace*{-\baselineskip}
\begin{tabularx}{\linewidth}{p{5cm} X}
\toprule
\bf Name  & \bf Possible values\\
\midrule
\textit{only first occurrence} (If false, use entities from the whole article, if true: ~\cite{voskarides-generating-2017}) &  $\{\mathbf{False}, True\}$ \\
\textit{max. \# co-occur entities} &  20 \\
\textit{only unambiguous rels query} &  $\{\mathbf{False}, True\}$ \\
%\textit{only unambiguous rels candidates} &  False \\
\textit{\# previous sentences to use} &  $\{0, \mathbf{1}\}$ \\
\textit{\# next sentences to use} &   $\{0, \mathbf{1}\}$ \\
\bottomrule
\end{tabularx}
\end{table}


How it works:
 \begin{itemize}
   \item positive examples are candidate triples identified in text spans that mention the query relationship instance. 

\item \textit{only first occurrence}: first occurrence strategy: we only take the first sentence in the Wikipedia article of the source entity that mentions the target entity ~\cite{voskarides-generating-2017} . If not activated, take the first \textit{max \# co-occur entities} co-occurring with the target entity.
        
      \item \textit{only unambigious rels query}, \textit{only unambigious rels candidates}: heuristic as in ~\citet{sorokin2017context}: if there is more than one relation, ignore it due to ambiguity. Different for query / candidates.
        
        \item \textit{\# previous sentences to use}, \textit{\# next sentences to use}
    
    \item \NV{Issue: if source to target are connected with multiple relations these don't end up in the candidates. (e.g. starsIn, awardWonfor movie). Solution: add all paths from source to target as relevant in distant supervision and get annotations./}
 
        
%       \item check \footnote{\url{http://xren7.web.engr.illinois.edu/sigmod17-StructNet.pdf}} and predecessor papers. e.g. pos patterns for matching relations?
%       \item Relation extraction 
%         \begin{itemize}
%             \item simple LM
%             \item unsupervised
%         \end{itemize}
  
 
%  \item fine-grained attributes: we could ask annotators to judge relevant facts to the relationship to double-check or to add more (``the second wife'' should add the other spouses) \NV{not for now}
  
\end{itemize}


==> neural-ranker.tex <==
%!TEX root = ./main.tex


\if0

\subsubsection{Representation learning}
\label{sec:neural-ranker}
%
%
In this section we describe the general framework of the neural fact ranker. First, we encode the relationship instance with a function $enc_{1}({r_i})$ and encode the candidate fact with a function $enc_{2}({f})$ (Section \ref{sec:fact-encoder}). We measure the similarity of the encoded relationship instance and the encoded candidate fact using a scoring function $u(enc_{1}(r_i),enc_{2}(f))$ (Section \ref{sec:scoring-func}).
%
Finally, we optimize the model using a loss function $L$ (Section \ref{sec:loss-func}).

%\subsubsection{Fact encoder}
%\label{sec:fact-encoder}

\paragraph{Entity representation} aggregate top-7 freebase types as in~\citet{das2017chains} (sum or maximum)

\if0
\begin{itemize}
    	\item long tail: impossible to learn good embeddings for millions of entities \NV{Motivate why not doing representation learning on the entities directly (huge \# entities, hard to learn embeddings directly)}

    \item aggregate top-7 freebase types as in~\citet{das2017chains} (sum or maximum)
	\item for mediators: use types if available or aggregate incoming/outgoing relations as in~\cite{voskarides-generating-2017}
	\item use in combination with entity embeddings  as in~\citet{das2017chains}. Only use popular entities.
	\item how to model that 2 entities are the same?
    	\begin{itemize}
          \item use distance from subject/object/mediator and use position features as in relation extraction (~\citet{zhang2017position}
          %\item constant during training or use trainable embeddings?
     \end{itemize}
\end{itemize}
\fi

\paragraph{Predicate representation} Embeddings initialized randomly. Reverse operation: transpose operation, as in ~\cite{guu2015traversing}

\if0
\begin{itemize}
     	\item how to model the reverse operation for predicates?
   		 \begin{itemize}
          \item transpose operation, as in ~\cite{guu2015traversing}
          \item add a special vector in the sequence
        \end{itemize}
\end{itemize}

\paragraph{Static encoder}
query and candidate separately: 
\begin{itemize}
	\item Concatenation of entities and predicates in each triple 
	\item MLP/CNN over triples (doesn't seem to help, we might be needing position features.)
\end{itemize}

\fi

\paragraph{Path encoder}

one RNN for the relationship instance.
candidate: one RNN per path from source to target, and aggregation of RNNs w/ attention mechanism\\

ToDo's
%\NV{
\begin{itemize}
    \item how to aggregate RNN vectors in one vector?
        \begin{itemize}
        \item  avg/log-sum-exp as in~\citet{das2017chains}, or
        \item  seq2seq-like attention
        \end{itemize}
\end{itemize}
%}


\subsubsection{Scoring function}
\label{sec:scoring-func}
Cosine similarity:
\begin{align}
	u(r_i,f;\theta) = cos(enc_{1}(r_i, \theta), enc_{2}(f, \theta))
\end{align}

\NV{ToDo's}
\begin{itemize}
	\item L1 similarity
	\item MLP
\end{itemize}


\NV{Discuss}
\begin{itemize}
	\item other pointwise loss functions (cross entropy, hinge loss)
	\item mean pairwise loss function 
	\item  max-margin loss for ranking as in \citet{barzilay2016semi}
	\item negative sampling
	\item positive class weighting to account for class imbalance
\end{itemize}


\if0
General non-priority todo's:
%\NV{
\begin{itemize}
 \item Pretrain with KG embeddings
 \item Wide \& deep to combine manually extracted features and embeddings~\footnote{\url{https://www.tensorflow.org/tutorials/wide_and_deep}}
 \item Dynamic KG embeddings? (He he ACL 2017, toutanova ACL 2016)   --- label/message propagation?
\item paper on modeling mediators (+)
\item We need to be able to return no results by (filtering by e.g. thresholding)
\end{itemize}
\fi

\fi

